GDC Cohort Copilot: An AI Copilot for Curating Cohorts from the Genomic Data Commons

The Genomic Data Commons (GDC) provides access to high quality, harmonized cancer genomics data through a unified curation and analysis platform centered around patient cohorts. While GDC users can interactively create complex cohorts through the graphical Cohort Builder, users (especially new ones) may struggle to find specific cohort descriptors across hundreds of possible fields and properties. However, users may be better able to describe their desired cohort in free-text natural language. We introduce GDC Cohort Copilot, an open-source copilot tool for curating cohorts from the GDC. GDC Cohort Copilot automatically generates the GDC cohort filter corresponding to a user-input natural language description of their desired cohort, before exporting the cohort back to the GDC for further analysis. An interactive user interface allows users to further refine the generated cohort. We develop and evaluate multiple large language models (LLMs) for GDC Cohort Copilot and demonstrate that our locally-served, open-source GDC Cohort LLM achieves better results than GPT-4o prompting in generating GDC cohorts. We implement and share GDC Cohort Copilot as a containerized Gradio app on HuggingFace Spaces, available at https://huggingface.co/spaces/uc-ctds/GDC-Cohort-Copilot. GDC Cohort LLM weights are available at https://huggingface.co/uc-ctds. All source code is available at https://github.com/uc-cdis/gdc-cohort-copilot.

==> macros.tex <==
\newcommand{\TODO}[1]{{\color{red}#1}}

%% ------------- Custom Author Notes -------------
%% see: https://tex.stackexchange.com/questions/577682/mix-number-and-symbols-on-thanks-marks
\makeatletter
\newcommand{\myfnsymbol}[1]{%
  \expandafter\@myfnsymbol\csname c@#1\endcsname
}
% Mapping of how the \thanks symbols will be interpreted sequentially
\newcommand{\@myfnsymbol}[1]{
  \ifcase #1% 0
  \or 1% 1 CTDS
  \or 2% 2 CS
  \or 3% 3 MSTP
  \or 4% 4 Biomed DS
  \or \TextOrMath{\textasteriskcentered}{*}% 5 cofirst
  \or \TextOrMath{\textdagger}{\dagger}% 6 corresponding
  \fi
}

% Just to make things explicit in the code what it means
\newcommand{\affilCTDS}{\@myfnsymbol{1}}
\newcommand{\affilCS}{\@myfnsymbol{2}}
\newcommand{\affilMSTP}{\@myfnsymbol{3}}
\newcommand{\affilBiomedDS}{\@myfnsymbol{4}}
\newcommand{\cofirst}{\@myfnsymbol{5}}
\newcommand{\corresponding}{\@myfnsymbol{6}}
\makeatother
